Distributionally Robust Offline Reinforcement Learning with Linear Function Approximation

Among the reasons hindering reinforcement learning (RL) applications to real-world problems, two factors are critical: limited data and the mismatch between the testing environment (real environment in which the policy is deployed) and the training environment (e.g., a simulator). This paper attempts to address these issues simultaneously with distributionally robust offline RL, where we learn a distributionally robust policy using historical data obtained from the source environment by optimizing against a worst-case perturbation thereof. In particular, we move beyond tabular settings and consider linear function approximation. More specifically, we consider two settings, one where the dataset is well-explored and the other where the dataset has sufficient coverage of the optimal policy. We propose two algorithms~-- one for each of the two settings~-- that achieve error bounds $\tilde{O}(d^{1/2}/N^{1/2})$ and $\tilde{O}(d^{3/2}/N^{1/2})$ respectively, where $d$ is the dimension in the linear function approximation and $N$ is the number of trajectories in the dataset. To the best of our knowledge, they provide the first non-asymptotic results of the sample complexity in this setting. Diverse experiments are conducted to demonstrate our theoretical findings, showing the superiority of our algorithm against the non-robust one.

==> entries/conclusions.tex <==
This paper studies the distributional robust offline RL with linear function approximation. Unlike the previous work, which projects the robust non-linear values into linear function space, we define the robust ambiguity in the feature space. Under the state-aggregation MDP and well-explored coverage assumptions, we propose a sample-efficient algorithm named DRVI-L. We also extend the result to the weaker coverage condition and model misspecification settings. Experiments show our proposed method can achieve proper robust behavior with fewer samples and fewer computing resources. We hope this work can be a cornerstone of the robust RL in large-scale practical problems.

==> entries/drvi.tex <==
\begin{algorithm}[ht]
    \caption{Distributionally Robust Value Iteration: Linear MDP (DRVI-L)}
    \label{alg:drvi}
   \begin{algorithmic}[1]
      \STATE {\bfseries Input:} $\underline{\beta}$, $ \mathcal{D}=\left\{\left(s_{h}^{\tau}, a_{h}^{\tau}, r_{h}^{\tau}\right)\right\}_{\tau, h=1}^{K, H} \text {. }$.
      \STATE {\bfseries Init:} $\widehat{V}_{H} = 0$.
      \FOR {step $h=H$ {\bfseries to} $1$}
      \STATE $\Lambda_{h}
      \leftarrow \sum_{\tau=1}^{K} \phi\left(s_{h}^{\tau}, a_{h}^{\tau}\right) \phi\left(s_{h}^{\tau}, a_{h}^{\tau}\right)^{\top}+\lambda I$
      \STATE $\widehat{\theta}_h \gets \Lambda_h^{-1} \left[\sum_{\tau=1}^{K} \phi(s_h^\tau, a_h^\tau) r_h^\tau \right]$
      \IF {$h=H$}
      \STATE $\widehat{w}_H \gets \widehat{\theta}_H$
      \ELSE 
      \STATE $\widehat{\psi}_h(s^{\prime}) \gets \Lambda^{-1}_h \left[\sum_{\tau=1}^{K} \phi(s_h^\tau, a_h^\tau) \mathds{1}(s_{h+1}^\tau = s^\prime)^\top \right]$, for $s^{\prime}\in \gS$
   %   \FOR {step $i=1$ {\bfseries to} $d$}
      \STATE $\widehat{w}_h^{[\cdot]} \gets \widehat{\theta}_h^{[\cdot]} + \max_{\beta\in[\underline{\beta}, \overline{\beta}]} \left\{ -\beta \log \left(\widehat{\psi}_{h}^{[\cdot]} e^{-\widehat{V}_{h+1} /\beta} \right) - \rho \beta \right\}$
   %   \ENDFOR
       \ENDIF
      \STATE $\bar{Q}_h(\cdot,\cdot) \gets \phi(\cdot,\cdot)^\top \widehat{w}_h $
     \STATE $\widehat{Q}_h(\cdot,\cdot) \gets \min\{\bar{Q}_h(\cdot,\cdot), H-h+1\}$
     \STATE $\widehat{\pi}_{h}(\cdot \mid \cdot) \leftarrow \arg \max _{\pi_{h}}\left\langle\widehat{Q}_{h}(\cdot, \cdot), \pi_{h}(\cdot \mid \cdot)\right\rangle_{\mathcal{A}}$
     \STATE $\widehat{V}_{h}(\cdot) \leftarrow\left\langle\widehat{Q}_{h}(\cdot, \cdot), \widehat{\pi}_{h}(\cdot \mid \cdot)\right\rangle_{\mathcal{A}}$
      \ENDFOR
   \end{algorithmic}
   \end{algorithm}

==> entries/lowerbound.tex <==
In this section, I will construct a lower bound following mengdi wang and zhihua zhou.

==> entries/pdrvi.tex <==
\begin{algorithm}[h]
    \caption{PDRVI-L}
    \label{alg:pdrvi}
   \begin{algorithmic}[1]
      \STATE {\bfseries Input:} $\underline{\beta}$, $ \mathcal{D}=\left\{\left(s_{h}^{\tau}, a_{h}^{\tau}, r_{h}^{\tau}\right)\right\}_{\tau, h=1}^{N, H}$.
      \STATE {\bfseries Init:} $\widehat{V}_{H} = 0$.
      \FOR {step $h=H$ {\bfseries to} $1$}
      \STATE $\Lambda_{h}
      \leftarrow \sum_{\tau=1}^{N} \phi\left(s_{h}^{\tau}, a_{h}^{\tau}\right) \phi\left(s_{h}^{\tau}, a_{h}^{\tau}\right)^{\top}+\lambda I$
      \STATE $\widehat{\theta}_h \gets \Lambda_h^{-1} \left[\sum_{\tau=1}^{N} \phi(s_h^\tau, a_h^\tau) r_h^\tau \right]$
      \IF {$h=H$}
      \STATE $\widehat{w}_H \gets \widehat{\theta}_H$
      \ELSE 
      \STATE $\widehat{\psi}_h(s^{\prime}) \gets \Lambda^{-1}_h \left[\sum_{\tau=1}^{N} \phi(s_h^\tau, a_h^\tau) \mathds{1}(s_{h+1}^\tau = s^\prime) \right]$, for $s^{\prime}\in \gS$
   %   \FOR {step $i=1$ {\bfseries to} $d$}
      \STATE $\bar{w}_{h,i} \gets \widehat{\theta}_{h,i} + \max_{\beta\in[\underline{\beta}, \infty]} \left\{ -\beta \log \left(\widehat{\psi}_{h,i}^{\top}(e^{-\widehat{V}_{h+1} /\beta} - 1) + 1 \right) - \rho \beta \right\}$
      \STATE $\widehat{w}_{h,i} \gets \max \left\{  \bar{w}_{h,i}, 0\right\}^+$, for $i \in [d]$
   %   \ENDFOR
       \ENDIF
      \STATE $\bar{Q}_h(\cdot,\cdot) \gets \phi(\cdot,\cdot)^\top \widehat{w}_h - \gamma_h \lVert \phi(\cdot, \cdot)\rVert_{\Lambda_h^{-1}}$
     \STATE $\widehat{Q}_h(\cdot,\cdot) \gets \bar{Q}_h(\cdot,\cdot)$
     \STATE $\widehat{\pi}_{h}(\cdot \mid \cdot) \leftarrow \arg \max _{\pi_{h}}\langle\widehat{Q}_{h}(\cdot, \cdot), \pi_{h}(\cdot \mid \cdot)\rangle_{\mathcal{A}}$
     \STATE $\widehat{V}_{h}(\cdot) \leftarrow\langle\widehat{Q}_{h}(\cdot, \cdot), \widehat{\pi}_{h}(\cdot \mid \cdot)\rangle_{\mathcal{A}}$
      \ENDFOR
   \end{algorithmic}
   \end{algorithm}

